FashionViL: Fashion-Focused Vision-and-Language Representation Learning

Large-scale Vision-and-Language (V+L) pre-training for representation learning has proven to be effective in boosting various downstream V+L tasks. However, when it comes to the fashion domain, existing V+L methods are inadequate as they overlook the unique characteristics of both the fashion V+L data and downstream tasks. In this work, we propose a novel fashion-focused V+L representation learning framework, dubbed as FashionViL. It contains two novel fashion-specific pre-training tasks designed particularly to exploit two intrinsic attributes with fashion V+L data. First, in contrast to other domains where a V+L data point contains only a single image-text pair, there could be multiple images in the fashion domain. We thus propose a Multi-View Contrastive Learning task for pulling closer the visual representation of one image to the compositional multimodal representation of another image+text. Second, fashion text (e.g., product description) often contains rich fine-grained concepts (attributes/noun phrases). To exploit this, a Pseudo-Attributes Classification task is introduced to encourage the learned unimodal (visual/textual) representations of the same concept to be adjacent. Further, fashion V+L tasks uniquely include ones that do not conform to the common one-stream or two-stream architectures (e.g., text-guided image retrieval). We thus propose a flexible, versatile V+L model architecture consisting of a modality-agnostic Transformer so that it can be flexibly adapted to any downstream tasks. Extensive experiments show that our FashionViL achieves a new state of the art across five downstream tasks. Code is available at https://github.com/BrandonHanx/mmf.

==> Figures/1-model_architecture.tex <==
\begin{figure}[t]
\begin{center}
\includegraphics[width=\linewidth]{Figures/overview.pdf}
\end{center}
\caption{Overview of the proposed FashionViL model architecture, consisting of an image encoder, a text encoder and a fusion encoder. Text encoder and fusion encoder share the same parameters\licheng{merge with Fig. 3}}
\label{fig:model_architecture}
\end{figure}

==> Figures/2-pretrian_tasks.tex <==
\begin{figure}[t]
\begin{center}
\includegraphics[width=\linewidth]{Figures/pretrain_tasks.pdf}
\end{center}
\caption{Illustrative diagram of six pre-training tasks}
\label{fig:pretrain_tasks}
\end{figure}
